Single Gaussian Process Method for Arbitrary Tokamak Regimes with a Statistical Analysis

Gaussian Process Regression (GPR) is a Bayesian method for inferring profiles based on input data. The technique is increasing in popularity in the fusion community due to its many advantages over traditional fitting techniques including intrinsic uncertainty quantification and robustness to over-fitting. This work investigates the use of a new method, the change-point method, for handling the varying length scales found in different tokamak regimes. The use of the Student's t-distribution for the Bayesian likelihood probability is also investigated and shown to be advantageous in providing good fits in profiles with many outliers. To compare different methods, synthetic data generated from analytic profiles is used to create a database enabling a quantitative statistical comparison of which methods perform the best. Using a full Bayesian approach with the change-point method, Mat\'ern kernel for the prior probability, and Student's t-distribution for the likelihood is shown to give the best results.

==> old_text.tex <==

    Gaussian process regression (GPR) is a non-parametric regression method that can fit arbitrarily spaced data, and it can account for uncertainties on the data.  It is a special type of Bayesian inference, and so we start by explaining the basics of Bayesian terminology.  We start with Bayes' theorem:
	\begin{equation}
	    K_{sek}\left(\psi,\psi'\right) = \theta_v e^ {-\frac{\left(\psi-\psi'\right)^2}{2\theta_l^2}}.
	\end{equation}
	
	A Gaussian process is extends the concept of a multivariate Gaussian distribution to a continuous domain. A Gaussian process is a stochastic process that the evaluation of the process at any collection of points in it's domain results in a multivariate Gaussian. A Gaussian process $GP\left(\mu\left(\psi\right),K\left(\psi,\psi'\right)\right)$ is uniquely define by a mean function $\mu\left(\psi\right)$ and a covariance kernel $K\left( \psi, \psi' \right)$. In this paper, we are interested in fitting flux function profiles, so the discussion here focuses of Gaussian process defined on the radial coordinate $\psi$, but the concepts naturally generalize to higher dimensions are more complex manifolds.
	
	A common Gaussian process has a zero mean $\mu=0$ and uses the squared exponential kernel (a.k.a. radial basis function):
	
	\begin{equation}
	    K_{sek}\left(\psi,\psi'\right) = \theta_v e^ {-\frac{\left(\psi-\psi'\right)^2}{2\theta_l^2}}.
	\end{equation}
	
	\noindent This Gaussian process is distribution over all smooth functions of $\psi$. Each function in the Gaussian process occurs with a certain probability that depends on the two hyper-parameters $\theta_v$ and $\theta_l$. The hyper-parameter $\theta_v$ characterizes how rapidly decreases as the function departs from the mean function ($0$ in this case), and $\theta_l$ characterizes the spatial correlation of the function at two points $\psi$ and $\psi'$. A kernel is \textit{stationary} is it only depends on the distance between two points $K\left(\psi,\psi'\right)=K\left(\left|\psi-\psi'\right|\right)$, otherwise the kernel is \textit{non-Stationary}.
	
	Gaussian Process Regression (GPR) uses Gaussian process to infer profiles from noisy data. A common framework for GPR using Bayesian analysis. The objective of Bayesian analysis is to calculate posterior probability distribution $p\left(f\left(\vec \psi_*\right)|\vec d, \vec \theta_{hp},\mathcal{I} \right)$. Here $f\left(\psi\right)$ is the underlying profile that is to be inferred and it is evaluated at the sampling locations $\vec \psi_* = \left[\psi_1, \psi_2, \dots \right]$ (GPR can also evaluate derivatives or integrals of function). The posterior distribution depends on the measured data $\vec d$, a given set of hyper-parameters $\theta_{hp}$, and prior knowledge $\mathcal{I}$.
	
	The direct calculation of the posterior is often challenging. Instead frequently it is more direct to calculate the likelihood of observing a set of measurements for a given profile $p\left(\vec d |f\left(\vec \psi_*\right),\vec \theta_{hp},\mathcal{I} \right)$. The likelihood distribution depends of forward model $S_m\left(f\right)$ that relates the profile to the noise free data and a model for the noise. A common choice for the noise is to assume normal noise result in a Gaussian likelihood distribution. 
	
	Bayes formula relates the posterior to the likelihood:
	\begin{equation}
	    p\left(f\left(
	    \vec \psi_*\right)|\ved d,\vec \theta_{hp}, \mathcal{I} \right) = \frac{p\left(\vec d |f\left(\vec \psi_*\right),\vec \theta_{hp}, \mathcal{I}\right)}{p\left(\vec d|\vec \theta_{hp}, \mathcal{I}\right)}GP\left(f\left(\vec \psi_*\right)|\vec \theta_{hp},\mathcal{I}\right),
	\end{equation}
	
	\noindent Bayes formula depends on two additional probability distributions. The prior probability $GP\left(f\left(\vec \psi_*\right)|\vec \theta_{hp},\mathcal{I}\right)$ quantifies the probability of each profile based solely on the hyper-parameters and other prior knowledge profile without any experimental data. As indicated by the notation, GPR assumes that the prior distribution is a Gaussian process. 
	The marginal likelihood (a.k.a. the evidence), $p\left(\vec d|\vec \theta_{hp}, \mathcal{I}\right)$, is the probability of measuring the data $\vec d$ for a given set of hyper-parameters and other prior knowledge.
	
	The hyper-parameters play an important role is GPR, and the choice of hyper-parameters requires special consideration. The simplest approaches is to pick reasonable values for the hyper-parameters that are learned from prior experiments. In this approach a large enough data set can overcome a bad choice of hyper-parameters. However, this approach suffers if underlying profile changes drastically in different experimental regimes or if the amount of measured data is limited, both of which are case here.
	
	A second approach is the \textit{Empirical Bayesian} where one tries to calculate the hyperparameters from the measured data by optimizing an objective function. For example, a common approach is to use the hyperparameters by maximize the marginal likelihood.
	
	The most rigorous approach is the \textit{Full Bayesian} approach which consider the posterior for all possible hyper-parameters. In this approach the hyper-parameters may be described by a hyper-prior $p\left(\theta_{hp}|\mathcal{I}\right)$ and one determines the probability
	\begin{equation}\label{eqn:fullbayes}
p\left(f\left(
	    \vec \psi_*\right)|\vec d,\mathcal{I} \right)=\int p\left(f\left(
	    \vec \psi_*\right)|\vec d,\vec \theta_{hp}, \mathcal{I} \right) p\left(
	   \vec \theta_{hp}| \mathcal{I} \right) d\vec \theta_{hp}
    \end{equation}
    
    As one moves up this hierarchy of approaches the accuracy of the calculation of the posterior distribution increases but so does the
    computational cost. When the forward model is a linear operator and noise is normal, analytic techniques can be used to calculate the posterior distribution for a given set of hyper-parameters. However, numerical techniques are needed to address nonlinear forward models, non-normal noise, and to evaluate the Full Bayesian posterior marginalized over the hyper-parameters (Eqn \ref{eqn:fullbayes}). \textif{Markov chain Monte Carlo} methods (MCMC) are a class algorithm that are used to calculate (sample) the posterior distribution that arises in various Bayesian approach.
    

	

	%\begin{figure}[b]
	%	\centering
	%	\includegraphics[width=\linewidth]{images/linear_device_schematic.pdf}%linear_device_schematic.jpg} %0.4
	%	\caption{A simple schematic of a linear device.  The magnetic field generated by the coils is roughly constant, pointing to the right.  The plasma source on the left produces a plasma that streams along the field-lines until impacting the target on the right.}
	%	\label{fig:linear_device}
	%\end{figure}
